The Fitness-Corrected Block Model, or how to create maximum-entropy data-driven spatial social networks

Models of networks play a major role in explaining and reproducing empirically observed patterns. Suitable models can be used to randomize an observed network while preserving some of its features, or to generate synthetic graphs whose properties may be tuned upon the characteristics of a given population. In the present paper, we introduce the Fitness-Corrected Block Model, an adjustable-density variation of the well-known Degree-Corrected Block Model, and we show that the proposed construction yields a maximum entropy model. When the network is sparse, we derive an analytical expression for the degree distribution of the model that depends on just the constraints and the chosen fitness-distribution. Our model is perfectly suited to define maximum-entropy data-driven spatial social networks, where each block identifies vertices having similar position (e.g., residence) and age, and where the expected block-to-block adjacency matrix can be inferred from the available data. In this case, the sparse-regime approximation coincides with a phenomenological model where the probability of a link binding two individuals is directly proportional to their sociability and to the typical cohesion of their age-groups, whereas it decays as an inverse-power of their geographic distance. We support our analytical findings through simulations of a stylized urban area.

==> related.tex <==
\section{Related Works}


Under the pressure of the COVID-19 pandemic, several simulation frameworks have been developed to provide realistic descriptions of the disease spread process on different spatial and temporal scales, from a single building to complex urban areas and even on a global scale. 
World-scale meta-population models and agent-based systems describing small and large areas can be informed by a variety of data sources. Census data and/or gridded population counts can be integrated to reconstruct populations that are statistically indistinguishable from real ones, including age, geographic distribution, education and wealth. The number and intensity of contacts in specific settings, such as workplaces, schools, or households, can be collected through surveys, questionnaires, diaries, and, if possible, supplemented with data obtained from digital technologies such as cell phones or wearable sensors ~\cite{Mossong-2008,eagle2009inferring,klepac2020contacts}. These data are then used to reconstruct contact matrices, individual or group schedules, and are widely used to reproduce synthetic interactions. ~\cite{del2007mixing,barrett2009generation}. 

In comparison, generative network models that can reproduce the characteristics of real-world social networks by incorporating information from data have received much less attention. The task of inferring a realistic distribution of social ties is quite challenging, since friendship ties can only be measured for a small subset of real-world networks, and the mechanism underlying tie formation, while thoroughly studied, is still far from being fully understood.
Ideally, the models should reproduce the main features of real-world social networks, well summarized in~\cite{kertesz2021modeling}. These networks show a heavy-tailed (e.g, lognormal) degree distribution, often with a finite cutoff in agreement with Dunbar's number. The transitivity of the networks is high, compared to a random graph model, as a consequence of the well-established principle that ``friends of my friends are my friends." Moreover, they show positive assortativity by degree and \emph{type}.
%The lack of available data about real-world social ties fostered the choice of rather simple models (\emph{e.g.}, Erdös-Rényi, Barabasi-Albert and Watts-Strogatz~\cite{newman2018networks}) which rely on just a few, easy to explain, assumptions. 
By quantitatively looking at ego networks, mobile phone networks,  and online social networks we now have a better  understanding of some of the peculiar feature of these networks and their underline mechanisms.
Education, wellness age and spatial proximity are regarded as critical element in the formation of friendship bonds~\cite{palla2007quantifying,HUANG2013969}, among these, age is probably the most studied possibly due to the fact that age-related data is actually available at different spatial scales~\cite{worldpop}. 
While there is wide evidence that geographical factors alone cannot explain the structure of real-world spatial social networks~\cite{scellato2011socio,liben2005geographic,herrera2015anatomy}, the dependence of friendship on distance is widely assumed to follow an inverse power-law with exponent $\beta\in[0.5, 2]$~\cite{lambiotte2008geographical,scellato2011socio,herrera2015anatomy,onnela2011geographic,liben2005geographic,illenberger2013role,walsh2011spatial,buchel2020cities} -- and this surprisingly holds even for online relationships~\cite{goldenberg2009distance}. In particular, $\beta<1$ seems to work better for short range contacts ($<20km$)~\cite{illenberger2013role} and for urban networks~\cite{walsh2011spatial}.
in line with sociological studies~\cite{krackhardt2003strength}, but contrary to other real-world networks~\cite{bernaschi2019spiders,newman2010networks}, such networks do not present very large hubs~\cite{onnela2007analysis,lambiotte2008geographical,herrera2015anatomy,liben2005geographic}.
Their degree distribution is right skewed and relatively long-tailed~\cite{herrera2015anatomy,liben2005geographic}, and it has been, at times, approximated by a power-law with a large ($5$ to $8$) exponent~\cite{onnela2007analysis,lambiotte2008geographical} or by a Lognormal distribution~\cite{illenberger2013role}.
Within cities, population density impacts on the frequency of close-range contacts, but usually not on the overall size of each person's network~\cite{buchel2020cities}.
While geographical proximity and community structure appear to be related~\cite{herrera2015anatomy,walsh2011spatial,buchel2020cities}, some authors argue that only small clusters ($<30$ members) are geographically bounded~\cite{onnela2011geographic} whereas the large ones may span across very large areas of a city~\cite{herrera2015anatomy}.

Defining simple models that capture all of these features is not an easy task.
Models designed to mimic the scale-free degree distribution emerging in many real networks, for instance, may fail to yield the expected clustering structure~\cite{cointet2007realistic,iskhakov2020local}. 
Exponential random graphs have been shown to overcome some of these limitations \cite{robins2007recent,daraganova2012networks}.

The community structure, which evidences the presence of a kind of homophily is a typical characteristic of real-world social networks and  Stochastic Block Models (SBMs) have been developed specifically to reproduce and study this feature. ~\cite{karrer2011stochastic,peixoto2014hierarchical}
In this type of network models the nodes are partitioned into disjoint sets named \textit{blocks} and the probability of an edge existing between two nodes depends on the blocks to which the two nodes belong.
The SBM and its generalization have gained their success in the last decades as they can be used to discover and understand the structure of a network, as well as for clustering purposes~\cite{mccallum2007topic,zhou2006probabilistic}.

Spatial network models are often obtained by incorporating vertices into a metric space; induced constraints can affect several properties of the network ~\cite{barthelemy2011spatial}. Introducing a penalty on "long" edges, which mimics a penalty in maintaining long-distance relationships, has an impact on clusters, path lengths, degree distributions, and more ~\cite{alizadeh2017generating}.

Recently, network instances having suitable features have been generated by means of the so-called \textit{random geometric} models~\cite{krioukov2010hyperbolic,boguna2010sustaining,serrano2008self}, where the popularity and similarity of the nodes depend on their position in some \emph{latent} metric space~\cite{papadopoulos2012popularity}.
%The distance function chosen for this space impacts on the properties of the obtained network.
Embedding the vertices into a hyperbolic disk~\cite{krioukov2010hyperbolic} has proved a way to obtain both high clustering and heavy-tailed degree distribution.








